A Critical Reflection on the Use of Toxicity Detection Algorithms in Proactive Content Moderation Systems

Toxicity detection algorithms, originally designed with reactive content moderation in mind, are increasingly being deployed into proactive end-user interventions to moderate content. Through a socio-technical lens and focusing on contexts in which they are applied, we explore the use of these algorithms in proactive moderation systems. Placing a toxicity detection algorithm in an imagined virtual mobile keyboard, we critically explore how such algorithms could be used to proactively reduce the sending of toxic content. We present findings from design workshops conducted with four distinct stakeholder groups and find concerns around how contextual complexities may exasperate inequalities around content moderation processes. Whilst only specific user groups are likely to directly benefit from these interventions, we highlight the potential for other groups to misuse them to circumvent detection, validate and gamify hate, and manipulate algorithmic models to exasperate harm.

==> summary.tex <==
\pagestyle{plain}
\setcounter{table}{0}
\captionsetup{labelformat=AppendixATables}

\begin{landscape}
\begin{longtable}{|>{\raggedright\arraybackslash}p{5cm}|>{\raggedright\arraybackslash}p{5cm}|>{\raggedright\arraybackslash}p{11cm}|}
\caption{Summary of Main Themes and Sub-Themes} \\
\hline
\textbf{Theme} & \textbf{Sub-theme} & \textbf{Summary} \\ \hline
\endfirsthead

\hline
\textbf{Theme} & \textbf{Sub-theme} & \textbf{Summary} \\ \hline
\endhead

\hline \multicolumn{3}{|r|}{\textit{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot

\textbf{Contextual factors impacting perceptions of toxicity and system effectiveness} 
& Conversational and interpersonal histories 
& The historical context of conversations, both personal and public, can influence the perception of toxicity. For example, language between friends may be considered toxic by an algorithm but not considered toxic by the individuals involved. \\ \cline{2-3} 

& Scale of abuse 
& The number of individuals involved in sending toxic messages and the audience size can amplify the harm caused. Messages part of network-level harassment~\citep{marwick2021morally} campaigns can be more harmful, even if individually they seem benign. \\ \cline{2-3} 

& Platform culture and affordances 
& Different platforms have distinct cultures and affordances, influencing the type and perception of toxic content. For instance, Twitter's algorithms could amplify and spread subtle forms of hate through trending topics. \\ \cline{2-3} 

& Social histories of oppression and power structures 
& Online content is influenced by offline socio-political power dynamics. Messages rooted in historical oppression (e.g., misogyny) need to be contextualised beyond their face value to understand their impact fully. \\ \hline

\textbf{End-user continuum of intention to send toxic messages} 
& The unaware and open to learning 
& Users who may unintentionally send toxic messages due to a lack of awareness. Proactive moderation can help educate and prevent future toxic behaviour. \\ \cline{2-3} 

& The emotionally triggered 
& Users who typically do not engage in toxic behaviour but may send harmful messages when emotionally triggered. These actions are often later regretted. \\ \cline{2-3} 

& Those using toxicity as a form of emotional arousal 
& Some users engage in toxic behaviour for emotional stimulation, such as fun or excitement. \\ \cline{2-3} 

& Those playing to an audience 
& Users who engage in toxic behaviour to gain attention or show off, especially in the presence of an audience. The presence of others can exacerbate their toxic actions. \\ \cline{2-3} 

& The determined and organised 
& Users with strong intentions to harm others, often part of coordinated efforts. These users are less likely to be deterred by moderation and may even adapt to circumvent it. \\ \hline

\textbf{Abuse and manipulation of systems with embedded toxicity models} 
& Validation 
& Toxicity scores provided by systems could unintentionally validate harmful behaviour, encouraging users to continue or escalate their actions. \\ \cline{2-3} 

& Gamification 
& Some users may treat toxicity scoring as a game, competing to achieve higher levels of toxicity or sharing their `scores' as a badge of honour. \\ \cline{2-3} 

& Model manipulation 
& Communities or users may attempt to manipulate toxicity detection models by providing false data, either to protect harmful content or to undermine the system's effectiveness. \\ \cline{2-3} 

& Circumvention 
& Users determined to send toxic messages may find ways to bypass the system, either by altering their language or using alternative methods of communication. \\ \hline

\label{tab:summary}
\end{longtable}
\end{landscape}

